Identities that represent powers of positive integers using multinomial coefficients

In this paper, we show combinatorial identities that represent powers of positive integers using multinomial coefficients, which do not come from the multinomial theorem and the multinomial Vandermonde's convolution.

==> Identities <==


@inproceedings{AjtaiSVP,
  title={The shortest vector problem in $L^2$ is NP-hard for randomized reductions},
  author={Ajtai, M.},
  booktitle={Proceedings of the 30th annual ACM symposium on Theory of computing},
  pages={10--19},
  year={1998},
  publisher = {ACM},
  series = {STOC '98}
}




@article{AlonFischerSzegedy2001,
title = {Parent-Identifying Codes},
journal = {Journal of Combinatorial Theory, Series A},
volume = {95},
number = {2},
pages = {349-359},
year = {2001},
author = {Alon, N. and Fischer, E. and Szegedy, M.}
}



@Inbook{Bai2015,
author = {Bai, S.
and Langlois, A.
and Lepoint, T.
and Stehl{\'e}, D.
and Steinfeld, R.},
editor = {Iwata, T.
and Cheon, J.H.},
title = {Improved Security Proofs in Lattice-Based Cryptography: Using the R{\'e}nyi Divergence Rather Than the Statistical Distance},
bookTitle = {Advances in Cryptology -- ASIACRYPT 2015},
year = {2015},
publisher = {Springer Berlin Heidelberg},
address = {Berlin, Heidelberg},
pages = {3--24},
abstract = {The R{\'e}nyi divergence is a measure of closeness of two probability distributions. We show that it can often be used as an alternative to the statistical distance in security proofs for lattice-based cryptography. Using the R{\'e}nyi divergence is particularly suited for security proofs of primitives in which the attacker is required to solve a search problem (e.g., forging a signature). We show that it may also be used in the case of distinguishing problems (e.g., semantic security of encryption schemes), when they enjoy a public sampleability property. The techniques lead to security proofs for schemes with smaller parameters, and sometimes to simpler security proofs than the existing ones.}
}




@techreport{vanEmdeBoas,
  title={Another NP-complete partition problem and the complexity of computing short vectors in a lattice},
  author={van Emde Boas, P.},
  year={1981},
  institution={Mathematics Department, University of Amsterdam},
  note = {81--04},
  type = {Technical Report}
}






@InProceedings{BCJ2011,
author="Becker, A.
and Coron, J. S.
and Joux, A.",
title="Improved Generic Algorithms for Hard Knapsacks",
booktitle="Advances in Cryptology -- EUROCRYPT 2011",
year="2011",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="364--385",
abstract="At Eurocrypt 2010, Howgrave-Graham and Joux described an algorithm for solving hard knapsacks of density close to 1 in time {\$}{\{}{\backslash}mathcal{\{}{\backslash}tilde O{\}}{\}}(2^{\{}0.337n{\}}){\$}and memory {\$}{\{}{\backslash}mathcal{\{}{\backslash}tilde O{\}}{\}}(2^{\{}0.256n{\}}){\$}, thereby improving a 30-year old algorithm by Shamir and Schroeppel. In this paper we extend the Howgrave-Graham--Joux technique to get an algorithm with running time down to {\$}{\{}{\backslash}mathcal{\{}{\backslash}tilde O{\}}{\}}(2^{\{}0.291n{\}}){\$}. An implementation shows the practicability of the technique. Another challenge is to reduce the memory requirement. We describe a constant memory algorithm based on cycle finding with running time {\$}{\{}{\backslash}mathcal{\{}{\backslash}tilde O{\}}{\}}(2^{\{}0.72n{\}}){\$}; we also show a time-memory tradeoff.",

}


@article{Vandermonde_type_identity_2014,
  title={A combinatorial contribution to the multinomial Chu-Vandermonde convolution},
  author={Belbachir, Hac{\`e}ne},
  journal={Les Annales RECITS},
  volume={1},
  pages={27-32},
  year={2014}
}





@article{pseudo_random_sets,
	abstract = {The notion of pseudo-randomness of subsets of {\{}1, 2,..., N{\}} is defined, and measures of pseudo-randomness are introduced. Then three special examples are studied. In two cases it turns out that the subset in question possesses strong pseudo-random properties, while the third example is a negative one.},
	author = {Dartyge, C{\'e}cile and S{\'a}rk{\"o}zy, Andr{\'a}s},
	date = {2007/06/01},
	date-added = {2025-12-06 15:46:39 +0900},
	date-modified = {2025-12-06 15:49:30 +0900},
	doi = {10.1007/s-10998-007-2183-y},
	id = {Dartyge2007},
	isbn = {1588-2829},
	journal = {Periodica Mathematica Hungarica},
	number = {2},
	pages = {183--200},
	rating = {0},
	read = {0},
	title = {On Pseudo-Random Subsets of the Set of the Integers Not Exceeding $N$},
	url = {https://doi.org/10.1007/s-10998-007-2183-y},
	volume = {54},
	year = {2007},
	bdsk-url-1 = {https://doi.org/10.1007/s-10998-007-2183-y}
}




@article{ChorRivest1988,
  title={A knapsack-type public key cryptosystem based on arithmetic in finite fields},
  author={Chor, B. and Rivest, R.L.},
  journal={IEEE Transactions on Information Theory},
  volume={34},
  memo = "number={5}",
  pages={901--909},
  year={1988},
  publisher={IEEE}
}



@book{ConwaySloaneBook1999,
title = {Sphere Packings, Lattices and Groups},
author = {Conway, J.H. and Sloane, N.J.A.},
series = {Grundlehren der mathematischen Wissenschaften},
volume = {290},
year = {1999},
publisher = {Springer, New York, NY}
}


@article{
CJLOSS,
author = {Coster,M.J. and Joux,A. and Lamacchia,B.A. and Odlyzko,A.M. 
and Schnorr,C.P. and Stern,J.},
title = {Improved low-density subset sum algorithms},
journal = {computational complexity},
volume = {2},
year = {1992},
pages = {111--128}
}


@article{EnumEncoding,
author = {T. Cover},
journal = {IEEE Transactions on Information Theory},
title = {Enumerative source encoding},
year = {1973},
volume = {19},
memo = "number = {1}",
pages = {73--77},
keywords = {Sequences;Source coding},
month = {January}
}


@book{Cover2006,
 author = {Cover, T.M. and Thomas, J.A.},
 title = {Elements of Information Theory (Wiley Series in Telecommunications and Signal Processing)},
 year = {2006},
 publisher = {Wiley-Interscience}
} 



@article{the_rank_of_a_random_matrix,
title = {The rank of a random matrix},
journal = {Applied Mathematics and Computation},
volume = {185},
number = {1},
pages = {689-694},
year = {2007},
issn = {0096-3003},
doi = {https://doi.org/10.1016/j.amc.2006.07.076},
url = {https://www.sciencedirect.com/science/article/pii/S0096300306009040},
author = {Xinlong Feng and Zhinan Zhang},
keywords = {Random matrix, Defective rank, Numerical rank, Condition number},
abstract = {This work is concerned with the numerical rank of matrix in the matrix computations. We conclude that a real random matrix has full rank with probability 1 and a rational random matrix has full rank with probability 1 too. Finally, the applications of the numerical matrix are given.}
}


@article{Furstenberg1977-SZ,
author = {Furstenberg, H.},
title = {Ergodic behavior of diagonal measures and a theorem of Szemerédi on arithmetic progressions},
journal = {Journal d'Analyse Math{\'e}matique},
volume = {31},
pages = {204-–256},
year = {1977}
}


@book{FurstenbergBook,
 author = {Furstenberg, H.},
 publisher = {Princeton University Press},
 title = {Recurrence in Ergodic Theory and Combinatorial Number Theory},
 year = {2014}
}





@book{GareyJohnson1979,
  title={Computers and intractability: A Guide to the Theory of NP-Completeness},
  author={Garey, M.R. and Johnson, D.S.},
  memo = "volume={29}",
  year={1979},
  publisher={WH Freeman and Company}
}


@article{generalizations_vandermonde_convolution_Gould_1956,
author = {H. W. Gould},
title = {Some Generalizations of Vandermonde's Convolution},
journal = {The American Mathematical Monthly},
volume = {63},
number = {2},
pages = {84--91},
year = {1956},
publisher = {Taylor ¥& Francis},
doi = {10.1080/00029890.1956.11988763},
URL = {https://doi.org/10.1080/00029890.1956.11988763
},
eprint = {https://doi.org/10.1080/00029890.1956.11988763
}
}



@article{Gowers2001,
author = {Gowers, W.},
title = {A new proof of Szemerédi's theorem},
journal = {GAFA, Geometric and functional analysis},
volume = {11}, 
pages = {465-–588},
year = {2001}
}


@book{concrete_mathematics_1994,
  title={Concrete Mathematics: A Foundation for Computer Science},
  author={Ronald Graham and Donald Knuth and Oren Patashnik},
  year={1994},
  publisher={Addison–Wesley}
}


@article{Green2003_CE_conj,
    author = {Green, B.},
    title = "{The Cameron–Erdős Conjecture}",
    journal = {Bulletin of the London Mathematical Society},
    volume = {36},
    number = {6},
    pages = {769-778},
    year = {2004},
    month = {11},
    abstract = "{ A subset A of the integers is said to be sum-free if there do not exist elements x, y, z ∈ A with x + y = z . It is shown that the number of sum-free subsets of \\{1,…, N \\} is O (2 N /2  ), confirming a well-known conjecture of Cameron and Erdős. 2000 Mathematics Subject Classification 11B75. }"
}




@article{GreenTao2008,
 author = {Green, B. and Tao, T.},
 journal = {Annals of Mathematics},
 number = {2},
 pages = {481--547},
 publisher = {Annals of Mathematics},
 title = {The Primes Contain Arbitrarily Long Arithmetic Progressions},
 volume = {167},
 year = {2008}
}





@inproceedings{HardyRamanujan1918,
  author = {Hardy, G.H. and Ramanujan, S.},
  year = {1918},
  title = {Asymptotic Formulae in Combinatory Analysis},
  booktitle = {Proceedings of the London Mathematical Society},
  publisher = {Wiley Online Library},
  memo = "issn = {0024-6115}",
  memo = "doi = {10.1112/plms/s2-17.1.75}",
  volume = {s2-17},
  memo = "month = {1}",
  pages = {75--115},
  memo = "number = {1}"
}





@Article{Impagliazzo1996,
author = {Impagliazzo,R. and Naor,M.},
title = {Efficient cryptographic schemes provably as secure as subset sum},
journal = {Journal of Cryptology},
year = {1996},
volume = {9},
memo = "number = {4}",
pages = {199--216}
}



@article{ino_kam_nai_ultra,
author = {Inoue, H. and Kamada,S. and Naito,K.}, 
title = {Simultaneous approximation problems 
of $p$-adic numbers 
and $p$-adic knapsack cryptosystems: 
Alice in $p$-adic numberland}, 
journal = {P-Adic Numbers, Ultrametric Analysis, and Applications}, 
volume = {8},
memo = "number = {4}",
pages = {312--324},
year = {2016},
publisher = {Springer}
}




@InProceedings{JouxGranKnapHash,
author = {Joux, A. and Granboulan, L.},
title = {A practical attack against knapsack based hash functions},
booktitle = {Advances in Cryptology -- EUROCRYPT 1994},
year = {1995},
publisher = {Springer Berlin Heidelberg},
address = {Berlin, Heidelberg},
pages = {58--66}
}



@article{laga-sap-np-hard,
author = {J. C. Lagarias},
journal = {SIAM Journal on Computing},
title = {The computational complexity of simultaneous Diophantine approximation problems},
year = {1985},
volume = {14},
memo = "number = {1}",
pages = {196-209}
}


@article{LO-attack,
author = {Lagarias,J.C. and Odlyzko,A.M.},
title = {Solving low-density subset sum problems},
journal = {Journal of the ACM},
volume = 32,
year = 1985,
pages = {229--246}
}




@article{Landau1903,
author = {Landau, E.},
title = {Neuer Beweis des Primzahlsatzes und Beweis des Primidealsatzes},
journal = {Mathematische Annalen},
volume = {56},
pages = {645--670},
year = {1903},
language = {Writen in German}
}





@inproceedings{IND_CPA_SubsetSum2010,
 author = {Lyubashevsky, V. and Palacio, A. and Segev, G.},
 title = {Public-key Cryptographic Primitives Provably As Secure As Subset Sum},
 booktitle = {Proceedings of the 7th International Conference on Theory of Cryptography},
 memo = "series = {TCC'10}",
 year = {2010},
 pages = {382--400},
 numpages = {19},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@book{MartinetBook2003,
author = {Martinet, J.},
title = {Perfect Lattices in Euclidean Spaces},
series = {A Series of Comprehensive Studies in Mathematics},
volume = {327},
year = {2003},
publisher = {Springer, Berlin, Heidelberg}
}

@article{MazoOdlyzko,
author = {Mazo, J.E. and Odlyzko, A.M.},
title = {Lattice points in high-dimensional spheres},
journal = {Monatshefte f{\"u}r Mathematik},
year = {1990},
memo="month = {March},
day = {01}",
volume = {110},
memo = "number = {1}",
pages = {47--61},
abstract = {Let N(x, n, $\alpha$) denote the number of integer lattice points inside the n-dimensional sphere of radius (an)1/2 with center at x. This numberN(x,n, $\alpha$) is studied for 
$\alpha$ fixed,n {\textrightarrow} ∞, andx varying. The average value (asx varies) ofN(x,n, 
$\alpha$) is just the volume of the sphere, which is roughly of the form (2 $\beta$e, $\alpha$)n/2. it is shown that the maximal and minimal values ofN (x,n, $\alpha$) differ from the everage by factors exponential inn, which is in contrast to the usual lattice point problems in bounded dimensions. This lattice point problem arose separately in universal quantization and in low density subset sum problems.}
}



@article{MerkleHellman, 
author = {Merkle, R.C. and Hellman, M.E.},
title = {Hiding information and signatures in trapdoor knapsacks},
journal = {IEEE Transactions on Information Theory},
volume = {24},
year = {1978},
pages = {525--530}
}


@book{SymmetricBilinearForms,
author = {Milnor, J. and Husemoller, D.},
title = {Symmetric Bilinear Forms},
series = {Ergebnisse der Mathematik und ihrer Grenzgebiete},
volume = {73},
year = {1973},
publisher = {Springer, Berlin, Heidelberg}
}






@article{probcoprime,
author = {Nymann, J.E.},
title = {On the Probability that $k$ Positive Integers are Relatively Prime},
journal = {Journal of Number Theory},
volume = {4},
pages = {469--473},
year = {1972}
}






@InProceedings{RelationsNonmalleability,
author = {Pass, R. and Shelat, A. and Vaikuntanathan, V.},
memo = "editor={Kurosawa, Kaoru}",
title = {Relations Among Notions of Non-malleability for Encryption},
booktitle = {Advances in Cryptology -- ASIACRYPT 2007},
year = {2007},
publisher = {Springer Berlin Heidelberg},
memo = "address={Berlin, Heidelberg}",
pages = {519--535},
abstract="Since its introduction in the early 90's, the notion of non-malleability for encryption schemes has been formalized using a number of conceptually different definitional approaches---most notably, the ``pragmatic'' indistinguishability-based approach and the ``semantical'' simulation-based approach. 
We provide a full characterization of these approaches and consider their robustness under composition."
}

@article{multinomial_identity_2022,
author = {Qi, Jiayue},
title = {An identity on multinomial coefficients},
year = {2022},
issue_date = {June 2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {56},
number = {2},
issn = {1932-2232},
url = {https://doi.org/10.1145/3572867.3572878},
doi = {10.1145/3572867.3572878},
abstract = {We introduce an identity on multinomial coefficients, as well as the proof for it.},
journal = {ACM Commun. Comput. Algebra},
month = nov,
pages = {68–71},
numpages = {4}
}

@book{Robert-p-adic,
author = {Robert,A.M.},
title = {A Course in $p$-adic Analysis},
publisher = {Springer-Verlag New York},
year = {2000}
}


@article{infodim,
author = {R{\'e}nyi,A.},
title = {On the dimension and entropy of probability distributions},
journal = {Acta Mathematica Academiae Scientiarum Hungarica},
year = {1959},
volume = {1},
pages = {193--215}
}



@article{multinomial_vandermonde_convolution_permanent_2021, title={Multinomial Vandermonde Convolution via Permanent}, volume={103}, DOI={10.1017/S000497272000115X}, number={3}, journal={Bulletin of the Australian Mathematical Society}, author={Rodtes, Kijti}, year={2021}, pages={353–361}}


@article{Roth1953AP,
author = {Roth, K.F.},
title = {On Certain Sets of Integers},
journal = {Journal of the London Mathematical Society},
volume = {s1-28},
number = {1},
pages = {104-109},
year = {1953}
}




@article{sapozhenko2008_CE_conj,
title = {The Cameron–Erdős conjecture},
author = {Sapozhenko, A.A.},
journal = {Discrete Mathematics},
volume = {308},
number = {19},
pages = {4361-4369},
year = {2008},
note = {Simonovits '06},
keywords = {Independent set, Sum-free set, Container method, Cameron–Erdős conjecture},
abstract = {A subset A of integers is said to be sum-free if a+b∉A for any a,b∈A. Let s(n) be the number of sum-free sets in interval [1,n] of integers. P. Cameron and P. Erdős conjectured that s(n)=O(2n/2). We show that s(n)∼c^02n/2 for even n and s(n)∼c^12n/2 for odd n, where c^0,c^1 are absolute constants, thereby proving the conjecture.}
}


@article{q_multinomial_vandermonde_convolution_SULANKE_1981,
title = {A generalized q-multinomial Vandermonde convolution},
journal = {Journal of Combinatorial Theory, Series A},
volume = {31},
number = {1},
pages = {33-42},
year = {1981},
issn = {0097-3165},
doi = {https://doi.org/10.1016/0097-3165(81)90051-0},
url = {https://www.sciencedirect.com/science/article/pii/0097316581900510},
author = {Robert A Sulanke},
abstract = {Bender's generalization of the q-binomial Vandermonde convolution is reformulated with weaker constraints. This and a similar convolution for q-multinomial coefficients are proved by interpreting the coefficients as generating functions that enumerate multidimensional lattice paths.}
}



@article{szemeredi1975,
  title={On sets of integers containing no $k$ elements in arithmetic progression},
  author={Szemer{\'e}di, E.},
  journal={Acta Arithmetica},
  volume={27},
  pages={199--245},
  year={1975},
  publisher={Instytut Matematyczny Polskiej Akademii Nauk}
}







@article{voronoi1908nouvelles,
  title={Nouvelles applications des param{\`e}tres continus {\`a} la th{\'e}orie des formes quadratiques. Premier m{\'e}moire. Sur quelques propri{\'e}t{\'e}s des formes quadratiques positives parfaites.},
  author={Voronoi, G.},
  journal={Journal f{\"u}r die reine und angewandte Mathematik},
  volume={1908},
  number={133},
  pages={97--102},
  year={1908},
  publisher={De Gruyter},
  language = {Writen in French}
}





